Claim-Dissector: An Interpretable Fact-Checking System with Joint Re-ranking and Veracity Prediction

We present Claim-Dissector: a novel latent variable model for fact-checking and analysis, which given a claim and a set of retrieved evidences jointly learns to identify: (i) the relevant evidences to the given claim, (ii) the veracity of the claim. We propose to disentangle the per-evidence relevance probability and its contribution to the final veracity probability in an interpretable way -- the final veracity probability is proportional to a linear ensemble of per-evidence relevance probabilities. In this way, the individual contributions of evidences towards the final predicted probability can be identified. In per-evidence relevance probability, our model can further distinguish whether each relevant evidence is supporting (S) or refuting (R) the claim. This allows to quantify how much the S/R probability contributes to the final verdict or to detect disagreeing evidence. Despite its interpretable nature, our system achieves results competitive with state-of-the-art on the FEVER dataset, as compared to typical two-stage system pipelines, while using significantly fewer parameters. It also sets new state-of-the-art on FAVIQ and RealFC datasets. Furthermore, our analysis shows that our model can learn fine-grained relevance cues while using coarse-grained supervision, and we demonstrate it in 2 ways. (i) We show that our model can achieve competitive sentence recall while using only paragraph-level relevance supervision. (ii) Traversing towards the finest granularity of relevance, we show that our model is capable of identifying relevance at the token level. To do this, we present a new benchmark TLR-FEVER focusing on token-level interpretability -- humans annotate tokens in relevant evidences they considered essential when making their judgment. Then we measure how similar are these annotations to the tokens our model is focusing on.

==> tables/he_performance.tex <==
\begin{tabular}{lllll}
\hline
\textbf{K$_1$+K$_2$} & \textbf{Recall} & \textbf{Recall}$_{MH}$ & \textbf{Recall}$_{MH_{ART}}$ & \textbf{\#SaI} \\ \hline
35+10          & 95.2            & 61.9              & 57.0                 & 269.6          \\
35+20          & 95.9            & 69.0              & 65.2                 & 309.0          \\
35+30          & 96.7            & 77.5              & 74.7                 & 388.6          \\
35+35          & 97.5            & 84.1              & 82.3                 & 506.7          \\
35+50          & 97.7            & 86.5              & 85.0                 & 624.3          \\
35+100         & 98.4            & 93.0              & 92.4                 & 1008.8         \\
100+100        & 98.6            & 93.4              & 92.7                 & 1431.0         \\ \hline
\end{tabular}
